Augmenting Automatic Speech Recognition Models with Disfluency Detection

Speech disfluency commonly occurs in conversational and spontaneous speech. However, standard Automatic Speech Recognition (ASR) models struggle to accurately recognize these disfluencies because they are typically trained on fluent transcripts. Current research mainly focuses on detecting disfluencies within transcripts, overlooking their exact location and duration in the speech. Additionally, previous work often requires model fine-tuning and addresses limited types of disfluencies. In this work, we present an inference-only approach to augment any ASR model with the ability to detect open-set disfluencies. We first demonstrate that ASR models have difficulty transcribing speech disfluencies. Next, this work proposes a modified Connectionist Temporal Classification(CTC)-based forced alignment algorithm from \cite{kurzinger2020ctc} to predict word-level timestamps while effectively capturing disfluent speech. Additionally, we develop a model to classify alignment gaps between timestamps as either containing disfluent speech or silence. This model achieves an accuracy of 81.62% and an F1-score of 80.07%. We test the augmentation pipeline of alignment gap detection and classification on a disfluent dataset. Our results show that we captured 74.13% of the words that were initially missed by the transcription, demonstrating the potential of this pipeline for downstream tasks.

==> sections/s2_related_word_old.tex <==

% \section{Related Work}
% \label{sec:related}
% Using an already established ASR system to improve the accuracy of a transcript has been investiaged by \cite{ma2023adapting}. Here, the authors attempted to fine-tune and soft-prompt Whisper to make the transcript more accurate. They achieved a WER improvement on the Linguskil dataset of 55.7\% (fine-tuning) and 50.6\% (soft-prompting) with 17 hours of training data. Additionally, they achieved a WER improvement on LibriSpeech of 15.5\% (fine-tuning) and 14.9\% (soft-prompting) with 10 hours of training data.

% Due to the fact that well-established commercial ASR systems are not universally accessible due to factors such as budget, target languages, and computational power, the authors of \cite{zhu2023transcription} developed a speech disfluency detection system that does not rely on existing ASR models. They employed structured state space sequence models (S4) and neural semi-Markov conditional random fields (semi-CRFs) for this purpose. These models receive the encoded audio features from a Wav2Vec2 feature encoder and calculate intervals where speech disfluencies occur. The authors of \cite{zhu2023transcription} achieved an absolute F1 improvement of 6.4\% (segment level) and 3.1\% (event level) on the PodcastFillers dataset.


==> sections/s3_approach_old.tex <==


% \section{Approach}
% \label{sec:methods}
% The approach consists of four steps. In the first step, a transcript is generated using a state-of-the-art ASR model. This transcript is then aligned with the audio using forced alignment. In this alignment, gaps should occur where speech was not transcribed because the words spoken at that time do not have an automatic generated equivalent. However, it is not certain that a gap contains untranscribed speech. People are known to pause when speaking. Therefore, all gaps above a certain length are checked for spoken language in the audio using a classification model. If this test is positive, the section of the audio corresponding to this gap is transcribed again. The resulting transcript is integrated into the initially generated transcript, resulting in a complete transcript.

% For the initial transcription of the audio, the Whisper-Large V3 model \cite{radford2023robust} was employed.



% \subsection{Forced Alignment}
% To align the transcript generated by Whisper to the audio, three approaches were employed. The cross-attention heads of Whisper exhibit a high degree of correlation with word-level timestamps. Consequently, is was initially attempted to use this as the primary alignment method. 
% % https://github.com/huggingface/transformers/blob/5346db168481640d1ce18f464470b102993049e7/src/transformers/models/whisper/generation_whisper.py#L157

% Another possibility is to achieve alignment through a network trained with a CTC loss function \cite{kurzinger2020ctc}. The CTC alignment algorithm can be modified to better align an incomplete transcript.

% \subsubsection{Modified CTC Alignment Algorithm}
% A problem that may arise when a transcript is incomplete is that the CTC algorithm extends the alignment around the incomplete transcript. This occurs because it is more likely to align a word for a longer duration than it is to align silence where something was being said. This is related to the fact that the emissions for a blank token in this part of the audio are very low, as something was spoken there.

% As a consequence, gaps in the alignment of the transcript may not occur where they should, which is undesirable for this application.

% To counteract this issue, the algorithm can be adjusted so that while creating the trellis, if the current label is a space token, the probability of staying on this label is the maximum of the probability acquired through the emissions and a predefined probability c. This modification incentives the algorithm to extend silence between words to some extent. However, this change encourages the algorithm to keep words short, since an alignment containing much silence gives a better score, and the predefined probability needs to be carefully chosen, as setting it too high may result in words being too short overall.


